The Ephemeral Threat: Assessing the Security of Algorithmic Trading Systems powered by Deep Learning

We study the security of stock price forecasting using Deep Learning (DL) in computational finance. Despite abundant prior research on the vulnerability of DL to adversarial perturbations, such work has hitherto hardly addressed practical adversarial threat models in the context of DL-powered algorithmic trading systems (ATS). Specifically, we investigate the vulnerability of ATS to adversarial perturbations launched by a realistically constrained attacker. We first show that existing literature has paid limited attention to DL security in the financial domain, which is naturally attractive for adversaries. Then, we formalize the concept of ephemeral perturbations (EP), which can be used to stage a novel type of attack tailored for DL-based ATS. Finally, we carry out an end-to-end evaluation of our EP against a profitable ATS. Our results reveal that the introduction of small changes to the input stock prices not only (i) induces the DL model to behave incorrectly but also (ii) leads the whole ATS to make suboptimal buy/sell decisions, resulting in a worse financial performance of the targeted ATS.

==> sections/fig_baseline.tex <==
\begin{figure*}[!htbp]
\centering
  % First Column
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{images/5Average_predicted_vs_actual_all_stocks.pdf}
    \caption{{\scriptsize \textbf{DL models.} Average RMSE=3.885}}
    \label{sfig:dl_baseline}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{images/5daily_returns.pdf}
    \caption{{\scriptsize \textbf{Daily Returns} of the ATS.}}
    \label{sfig:daily_returns}
  \end{subfigure}

  % Second Column
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{images/cumulative_returns.pdf}
    \caption{{\scriptsize \textbf{Daily Returns (cumulative).}}}
    \label{sfig:daily_returns_cumulative}
  \end{subfigure}\hfill
  \begin{subfigure}[b]{0.48\textwidth}
    \centering
    \includegraphics[width=0.99\linewidth]{images/5sharpe_ratio.pdf}
    \caption{{\scriptsize \textbf{Sharpe Ratio.} Mostly above 1.}}
    \label{sfig:sharpe_ratio}
  \end{subfigure}

\caption{\textbf{Baseline System.} \textmd{\footnotesize We show the profitability of our self-developed ATS. The DL models effectively predict the future closing price of the stocks in the portfolio (Fig.~\ref{sfig:dl_baseline}). The ATS uses these predictions to apply the moving average crossover trading strategy, leading to financial decisions that net a profit over-time (Fig.~\ref{sfig:daily_returns_cumulative}). Such a positive gain is reflected by the sharpe ratio consistently above 0 (Fig.~\ref{sfig:sharpe_ratio}).}}
\label{fig:baseline}
\end{figure*}


==> sections/results_figures.tex <==

\begin{figure*}[!htbp]
\centering
    \begin{subfigure}[!htbp]{0.65\columnwidth}
        \centering
        \frame{\includegraphics[width=0.99\columnwidth]{images/google_stock_prediction_attackw90.pdf}}
        \vspace{-1mm}
        \caption{{\scriptsize \textbf{DL predictor.} \textmd{We introduce a tiny perturbation (dotted line) on the closing price of GOOGL on day 90. The EP leads the LSTM, when predicting the closing price for day 91, to output a different value. The EP ``disappears'' on day 91.}}}
        \label{sfig:attack_ml}
    \end{subfigure}\hfill
    \begin{subfigure}[!htbp]{0.65\columnwidth}
        \centering
        \frame{\includegraphics[width=0.99\columnwidth]{images/cumulative_returns_comparison_attack_on_day_90 (5).pdf}}
        \vspace{-1mm}
        \caption{{\scriptsize \textbf{Whole ATS.} \textmd{We measure the effects of the EP introduced on day 90. Starting from the following day, the Sharpe Ratio of the ATS drops (inducing a monetary loss) substantially w.r.t. the baseline---despite the EP affecting only one day.}}}
        \label{sfig:attack_ats}
    \end{subfigure}\hfill
    \begin{subfigure}[!htbp]{0.65\columnwidth}
        \centering
        \frame{\includegraphics[width=0.99\columnwidth]{images/NRCR_Density_Function_Normalized.pdf}} 
        \vspace{-1mm}
        \caption{{\scriptsize \textbf{Normalized Relative Cumulative Return (NRCR)} \textmd{It is a cumulative return relative to the baseline cumulative return normalized by the attack duration. Ones extra line one extra line to reach four lines}}}
        \label{sfig:nrcr}
    \end{subfigure}
    \vspace{-2mm}
    \caption{\textbf{Exemplary results of an EP.}
    \textmd{\footnotesize We showcase what happens if a DL predictor and overarching ATS are targeted by some of our proposed EP. The blue line represents the baseline performance (y-axis), whereas the others represent the effects of various EPs over our test timeframe (x-axis).}}
    \label{fig:attack}
    \vspace{-3mm}
\end{figure*}



